Customizable Perturbation Synthesis for Robust SLAM Benchmarking

Robustness is a crucial factor for the successful deployment of robots in unstructured environments, particularly in the domain of Simultaneous Localization and Mapping (SLAM). Simulation-based benchmarks have emerged as a highly scalable approach for robustness evaluation compared to real-world data collection. However, crafting a challenging and controllable noisy world with diverse perturbations remains relatively under-explored. To this end, we propose a novel, customizable pipeline for noisy data synthesis, aimed at assessing the resilience of multi-modal SLAM models against various perturbations. This pipeline incorporates customizable hardware setups, software components, and perturbed environments. In particular, we introduce comprehensive perturbation taxonomy along with a perturbation composition toolbox, allowing the transformation of clean simulations into challenging noisy environments. Utilizing the pipeline, we instantiate the Robust-SLAM benchmark, which includes diverse perturbation types, to evaluate the risk tolerance of existing advanced multi-modal SLAM models. Our extensive analysis uncovers the susceptibilities of existing SLAM models to real-world disturbance, despite their demonstrated accuracy in standard benchmarks. Our perturbation synthesis toolbox, SLAM robustness evaluation pipeline, and Robust-SLAM benchmark will be made publicly available at https://github.com/Xiaohao-Xu/SLAM-under-Perturbation/.

==> figs/fig_case_study_stereo_slam_euroc_baseline_perturb.tex <==
\begin{figure*}[t]
	\centering
\includegraphics[width=\textwidth]{figures/case_study_stereo_slam_euroc_baseline_perturb.pdf} 
	\caption{\textbf{Effect of perturbations on the stereo camera baseline and inter-camera transformation matrix in a stereo SLAM system.} We introduce random noise $\eta$ along the axis of the stereo camera baseline length. The noise is sampled from a Gaussian distribution with zero mean and variance $\sigma^2$, represented as $\eta \sim \mathcal{N}(0, \sigma^2)$. We illustrate (\textbf{a}) the clean setting without noise and two perturbed settings with two severity levels of noise: (\textbf{b}) $\sigma=0.001$ [m] and (\textbf{c}) $\sigma=0.01$ [m] (with three runs each). For this analysis, we provide a qualitative comparison using the EuRoC~\cite{Burri25012016} dataset. The predefined camera baseline length is set to 0.1 meters, and the stereo camera input setting of the ORBSLAM3~\cite{orbslam3} model is employed. Additionally, we include quantitative metrics to quatify trajectory estimation error, \textit{i.e.}, 'Trans', 'Scale', and 'TransGT', with all values expressed in centimeters. For more details about these metrics, please refer to the ORBSLAM3~\cite{orbslam3} literature.} 
	\label{fig:stereo-slam-baseline-perturb}
\end{figure*}

==> figs/fig_fast_motion_correlation.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/all_boxplots.pdf} 
	\caption{\textit{Faster Motion} perturbation on the performance for splatam}%\vspace{-2mm}
	\label{fig:recon-fast-motion}
\end{figure}

==> figs/fig_image_perturbation_weather.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.49\textwidth]{figures/carla_weather_effects.pdf} 
	\caption{Illustration of image-level corruption for outdoor scenes empowered via CARLA simulator~\cite{dosovitskiy2017carla}. Columns represent different realistic weather effects, while rows show varying severity levels.}%\vspace{-2mm}
	\label{fig:sensor-corruption-weather}
\end{figure}

==> figs/fig_qualitative_result_faster_motion.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{figures/fast_motion_splatam_all_boxplots.pdf} 
	\caption{Qualitative result of the effect of \textit{Faster Motion} perturbation on the performance for each scene in the Replica Dataset. The x-axis denotes the speed-up ratio. The y-axis denotes ATE RMSE in the log scale. \textcolor{red}{Currently, we only show the result pf Splatam. More of them will be added later. Detailed values please refer to the appendix.TODO, compare among methods}}%\vspace{-2mm}
\label{fig:faster-motion-splatam-compare}
\end{figure}

==> figs/fig_result_fast_motion.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figures/qualitative_result_coslam_faster_motion.png} 
	\caption{Effect of \textit{Faster Motion} perturbation on the performance for each scene in the Replica Dataset. We visualize the 3D point cloud reconstruction of an environment, accompanied by graphs comparing predicted trajectory (in blue) with ground truth trajectory (in black).}%\vspace{-2mm}
	\label{fig:faster-motion-coslam-qualitative}
\end{figure}

==> figs/fig_simulator_pipeline_bak.tex <==
\begin{figure*}[ht]
	\centering	\includegraphics[width=0.8\textwidth]{figures/RobuSLAM_Simulation_Pipeline.pdf} 
	\caption{\textbf{Robust-SLAM Simulation Pipeline Overview.} (a) Data Synthesis: Modular, robot-centric framework couples robot dynamics with advanced physics and sensor configurations for accurate 3D scene-derived sensor streams. (b) Perturbation: Dual-layered composers introduce variability in trajectory and sensor data. (c) SLAM Evaluation: Synthesized and perturbed data facilitates rigorous SLAM benchmarking. }%\vspace{-2mm}
	\label{fig:pipeline}
\end{figure*}

==> tables/table_sensor_perturb_performance_bak.tex <==

\begin{table*}[t]
\caption{Performance (ATE RMSE [m]) under image perturbation in the static (top) and dynamic (bottom) perturbation mode. For cases where no final trajectory is produced (e.g., due to tracking loss or out of GPU memory ($>24GB$)), we assign an ATE of 1.0 and calculate the average ATE for each perturbation type. These cases are denoted with an "F" at the end of the result.}
\label{tab:sensor_perturb_static}
\centering\setlength{\tabcolsep}{0.8mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cc|cccc|cccc|cccc|cccc}
    \toprule \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Clean}}&  \multicolumn{2}{|c|}{\textbf{Perturbed}}  & \multicolumn{4}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Environmental Interference}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{5-8} \cmidrule{9-12} \cmidrule{13-16} \cmidrule{17-20}
    &  & \textbf{Mean} & \textbf{Max}  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{20}{c}{Static Perturbation Mode for Monocular Setting SLAM Models}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
    GO-SLAM~\cite{zhang2023goslam} & $0.0039$ & $0.000$  & $0.000$ & $0.0151$ & $0.0052$ & $0.0052$ & $0.0089$ & $0.0776$ & $0.0456$ & $0.0296$ & $0.0190$ & $0.2157$ & $0.7207$ & $0.1921$ & $0.0859$ & $0.0046$ & $0.0047$ & $0.0095$ & $0.0046$ 
   
    \\ \midrule
        \multicolumn{20}{c}{Static Perturbation Mode for RGBD Setting SLAM Models}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Nice-SLAM~\cite{niceslam}& $0.0147$ & $0.000$ & $0.000$  & $0.0307$ & $0.0151$ & $0.0161$ & $0.0188$ & $0.0254$ & $0.0377$ & $0.0353$ & $0.0151$ & $0.0186$ & $0.0160$ & $0.0323$ & $0.0320$ & $0.0654$ & $0.0161$ & $0.0150$ & $0.0145$
    \\
    CO-SLAM~\cite{coslam}& $0.0090$ & $0.000$ & $0.000$  & $0.0115$ & $0.0096$ & $0.0097$ & $0.0097$ & $0.0125$ & $0.0101$ & $0.0099$ & $0.0105$ & $0.0118$ & $0.0113$ & $0.0104$ & $0.0098$ & $0.0103$ & $0.0112$ & $0.0094$ & $0.0094$

    \\

    GO-SLAM~\cite{zhang2023goslam} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    Splatam-S~\cite{keetha2023splatam}& $0.0045$ & $0.000$ & $0.000$ & $0.0142$ & $0.0054$  & $0.0048$ & $0.0049$ & $0.0056$ & $0.0053$ & $0.0045$ & $0.0049$ & $0.0086$ & $0.0063$ & $0.0049$ & $0.0051$ & $0.0037$ & $0.0121$ & $0.0043$ & $0.0049$  
    \\
    \bottomrule \bottomrule
    \end{tabular}
}
\end{table*}


\begin{table*}[t]
\caption{Performance (ATE RMSE [m]) under image perturbation in the dynamic perturbation mode.}
\label{tab:sensor_perturb_dynamic}
\centering\setlength{\tabcolsep}{0.8mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cc|cccc|cccc|cccc|cccc}
    \toprule \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Clean}}&  \multicolumn{2}{|c|}{\textbf{Perturbed}}  & \multicolumn{4}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Environmental Interference}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{5-8} \cmidrule{9-12} \cmidrule{13-16} \cmidrule{17-20}
    &  & \textbf{Mean} & \textbf{Max}  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{20}{c}{Dynamic Perturbation Mode for Monocular Setting SLAM Models}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\    
    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ 
    \\
        GO-SLAM~\cite{zhang2023goslam} & $0.0039$ & $0.000$ & $0.000$ & $0.0155$ & $0.0065$   & $0.0060$ & $0.0090$  & $0.0509$ & $0.0253$ & $0.0396$ & $0.0158$ & $0.2668$ & $0.7395$& $0.2254$  & $0.0474$ & $0.0066$ & $0.0050$ & $0.0298$ & $0.0044$ 
    \\
    \midrule
        \multicolumn{20}{c}{Dynamic Perturbation Mode for RGBD Setting SLAM Models}  \\ \midrule
    ORBSLAM3~\cite{orbslam3} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\

    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ 
    \\
    IMAP~\cite{imap} & $0.1209$ & $0.000$ & $0.000$ & $0.1243$ & $0.1042$ & $0.2149$  & $0.1221$ & $0.1354$ & $0.1170$ & $0.1967$ & $0.1576$ & $0.2279$ & $0.2873$ & $0.2412$ & $0.1528$ & $0.2141$ & $0.2576$ & $0.1607$ & $0.0955$ 
    \\
    Nice-SLAM~\cite{niceslam}& $0.0147$ & $0.000$ & $0.000$  & $0.0157$ & $0.0252$ & $0.0359$ & $0.0211$ & $0.0288$ & $0.0409$ & $0.0146$ & $0.0155$ & $0.0167$ & $0.0211$ & $0.0197$ & $0.0187$ & $0.0206$ & $0.0155$ & $0.0146$ & $0.0170$
    \\
    CO-SLAM~\cite{coslam}& $0.0090$ & $0.000$ & $0.000$ & $0.0107$ & $0.0095$ & $0.0115$ & $0.0093$ & $0.0106$ & $0.0103$ & $0.0102$ & $0.0098$ & $0.0117$ & $0.0116$ & $0.0111$ & $0.0109$ & $0.0106$ & $0.0111$ & $0.0095$ & $0.0097$
    \\
 GO-SLAM~\cite{zhang2023goslam} & $0.0046$ & $0.000$  & $0.000$ & $0.0130$ & $0.0057$ & $0.0055$ & $0.0078$ & $0.0185$ & $0.0117$ & $0.0139$ & $0.0098$ & $0.1685$ & $0.2213$ & $0.0637$ & $0.0166$ & $0.0051$ & $0.0052$ & $0.0092$ & $0.0049$ 
    \\ 
    Splatam-S~\cite{keetha2023splatam}& $0.0045$ & $0.000$ & $0.000$ & $0.0195$ & $0.0053$  & $0.0052$ & $0.0050$ & $0.0058$ & $0.0072$ & $0.0043$ & $0.0067$ & $0.0062$ & $0.0063$ & {$0.0469$F} & $0.0040$ & $0.0054$ & $0.0096$ & $0.0045$ & $0.0046$  
    \\
    \bottomrule  \bottomrule
    \end{tabular}
}
\end{table*}





\begin{table*}[t]
\caption{Performance (ATE RMSE [m] ($\downarrow$)) under static (\textbf{Top}) and dynamic (\textbf{Bottom}) image perturbations. }
\label{tab:image_perturb}
\centering\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|cc|cccc|cccc|cccc|cccc}
    \toprule \toprule
     \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Clean}}&  \multicolumn{2}{|c|}{\textbf{Perturbed}}  & \multicolumn{4}{|c|}{\textbf{Blur Effect}} & \multicolumn{4}{c|}{\textbf{Noise Effect}} & \multicolumn{4}{c|}{\textbf{Environmental Interference}}  & \multicolumn{4}{c}{\textbf{Post-processing Effect}} 
    \\ \cmidrule{5-8} \cmidrule{9-12} \cmidrule{13-16} \cmidrule{17-20}
    &  & \textbf{Mean} & \textbf{Max}  & \textbf{Motion} & \textbf{Defocus} & \textbf{Gaussian} & \textbf{Glass} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Impulse} & \textbf{Speckle} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Spatter} & \textbf{Bright} & \textbf{Contra.} & \textbf{Jpeg}  & \textbf{Pixelate}
    \\\midrule\midrule
    \multicolumn{20}{c}{\textbf{Static Perturbation} Mode for \textbf{Monocular} SLAM Models}  \\ \midrule
   %  VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$     \\
    ORBSLAM3~\cite{orbslam3} & $0.0145$ & $0.763F$ & $1.4284$  & $0.891F$ & $0.535F$ & $0.505F$ & $0.797F$ & $0.917F$ & $0.969F$ & $1.000F$ & $0.923F$ & $0.629F$ & $0.917F$ & $1.000F$ & $0.719F$ & ${0.0265}$ & $0.612F$ & $1.000F$ & $0.768F$ 
    \\    
    GO-SLAM~\cite{zhang2023goslam} & $\textbf{0.0039}$ & $\textbf{0.0903}$  & $\textbf{0.7207}$ & $\textbf{0.0151}$ & $\textbf{0.0052}$ & $\textbf{0.0052}$ & $\textbf{0.0089}$ & $\textbf{0.0776}$ & $\textbf{0.0456}$ & $\textbf{0.0296}$ & $\textbf{0.0190}$ & $\textbf{0.2157}$ & $\textbf{0.7207}$ & $\textbf{0.1921}$ & $\textbf{0.0859}$ & $\textbf{0.0046}$ & $\textbf{0.0047}$ & $\textbf{0.0095}$ & $\textbf{0.0046}$ 
   
    \\ \midrule
        \multicolumn{20}{c}{\textbf{Static Perturbation} Mode for \textbf{RGBD} SLAM Models}  \\ \midrule
 %    VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$   \\
    ORBSLAM3~\cite{orbslam3} & $0.0823$ & $0.476F$ & $1.1606$ & $0.300F$ & $0.340F$ & $0.292F$ & $0.211F$ & $0.470F$ & $0.433F$ & $0.591F$ & $0.351F$ & $0.397F$ & $0.640F$ & $0.795F$ & $0.508F$ & $0.0649$ & $0.527F$ & $1.00F$ & $0.7034$
    \\
    IMAP~\cite{imap} & $0.1209$ & $0.1568$ & $0.3831$ & $0.1424$ & $0.1671$ & $0.1811$ & $0.0672$ & $0.0278$ & $0.0779$ & $0.1710$ & $0.1087$ & $0.1913$ & $0.1316$ & $0.1665$ & $0.1473$ & $0.1903$ & $0.3831$ & $0.1884$ & $0.1669$  
    \\
    Nice-SLAM~\cite{niceslam}& $0.0147$ & $0.0253$ & $0.0377$  & $0.0307$ & $0.0151$ & $0.0161$ & $0.0188$ & $0.0254$ & $0.0377$ & $0.0353$ & $0.0151$ & $0.0186$ & $0.0160$ & $0.0323$ & $0.0320$ & $0.0654$ & $0.0161$ & $0.0150$ & $0.0145$
    \\
    CO-SLAM~\cite{coslam}& $0.0090$ & $0.0104$ &  $\textbf{0.0125}$  & $\textbf{0.0115}$ & $0.0096$ & $0.0097$ & $0.0097$ & $0.0125$ & $0.0101$ & $0.0099$ & $0.0105$ & $0.0118$ & $0.0113$ & $0.0104$ & $0.0098$ & $0.0103$ & $0.0112$ & $0.0094$ & $0.0094$

    \\

    GO-SLAM~\cite{zhang2023goslam} & $0.0046$ & $0.0574$ &$0.6271$ & $0.0135$ & $\textbf{0.0052}$ & ${0.0052}$ & $0.0090$ & $0.0169$ & $0.0140$ & $0.0171$ & $0.0100$ & $0.1211$ & $0.6271$ & $0.0416$ & $0.0164$ & $0.0047$ & $\textbf{0.0054}$ & $0.0065$ & $0.0050$ 
    \\
    SplaTAM-S~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $\textbf{0.0062}$ & $0.0160$ & $0.0160$ & $\textbf{0.0052}$  & $\textbf{0.0049}$ & $\textbf{0.0048}$ & $\textbf{0.0054}$ & $\textbf{0.0050}$ & $\textbf{0.0044}$ & $\textbf{0.0051}$ & $\textbf{0.0085}$ & $\textbf{0.0063}$ & $\textbf{0.0048}$ & $\textbf{0.0051}$ & $\textbf{0.0038}$ & $0.0133$ & $\textbf{0.0044}$ & $\textbf{0.0048}$  
    \\  \midrule
        \multicolumn{20}{c}{\textbf{\textit{Survival Upper-bound:}} The highest expected performance (min ATE) attainable using all advanced models.}  \\ \midrule
      min ATE  & \multirow{3}{*}{$0.0045$} & \multirow{3}{*}{${0.0056}$}   & {${0.0115}$} & $0.0115$ & $0.0052$  & $0.0049$ & $0.0048$ & $0.0054$ & $0.0050$ & $0.0044$ & $0.0051$ & $0.0085$ & $0.0063$ & $0.0048$ & $0.0051$ & $0.0038$ & $0.0054$ & $0.0044$ & $0.0048$  
    \\ \cmidrule{5-8}\cmidrule{9-12}\cmidrule{13-16}\cmidrule{17-20}
     mean(min ATE)& &  & {0.0066}  &  \multicolumn{4}{c|}{${0.0066}$}&  \multicolumn{4}{c|}{$0.0050$}&  \multicolumn{4}{c|}{$0.0062$} &  \multicolumn{4}{c}{$0.0046$}
    \\ 
       \midrule     \midrule
    \multicolumn{20}{c}{\textbf{Dynamic Perturbation} Mode for \textbf{Monocular} SLAM Models}  \\ \midrule
  %   VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$  & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$  & $0.000$ & $0.000$   \\
    ORBSLAM3~\cite{orbslam3} & $0.0145$ & $0.854F$ & $1.2481$  & $0.925F$ & $0.506F$ & $0.760F$ & $0.813F$ & $1.000F$ & $1.000F$ & $1.000F$ & $0.885F$ & $0.751F$ & $1.000F$ & $1.000F$ & $1.000F$ & $0.0517$ & $1.000F$ & $1.000F$ & $0.718F$ 
    \\    
        GO-SLAM~\cite{zhang2023goslam} & $\textbf{0.0039}$ & $\textbf{0.0933}$ & $\textbf{0.7395}$ & $\textbf{0.0155}$ & $\textbf{0.0065}$   & $\textbf{0.0060}$ & $\textbf{0.0090}$  & $\textbf{0.0509}$ & $\textbf{0.0253}$ & $\textbf{0.0396}$ & $\textbf{0.0158}$ & $\textbf{0.2668}$ & $\textbf{0.7395}$& $\textbf{0.2254}$  & $\textbf{0.0474}$ & $\textbf{0.0066}$ & $\textbf{0.0050}$ & $\textbf{0.0298}$ & $\textbf{0.0044}$ 
    \\
    \midrule
        \multicolumn{20}{c}{\textbf{Dynamic Perturbation} Mode for \textbf{RGBD} SLAM Models}  \\ \midrule
  %   VINS-Fusion~\cite{qin2018vins} & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$ & $0.000$     \\
   ORBSLAM3~\cite{orbslam3} & $0.0823$ & $0.594F$ & $1.0629$  & $0.279F$ & $0.303F$ & $0.0515$ & $0.1680$ & $0.508F$ & $0.513F$ & $0.755F$ & $0.262F$ & $0.659F$ & $0.256F$ & $0.876F$ & $0.753F$ & $0.0660$ & $0.751F$ & $1.000F$ & $0.756F$ 
    \\
    IMAP~\cite{imap} & $0.1209$ & $0.1756$ & $0.2873$ & $0.1243$ & $0.1042$ & $0.2149$  & $0.1221$ & $0.1354$ & $0.1170$ & $0.1967$ & $0.1576$ & $0.2279$ & $0.2873$ & $0.2412$ & $0.1528$ & $0.2141$ & $0.2576$ & $0.1607$ & $0.0955$ 
    \\
    Nice-SLAM~\cite{niceslam}& $0.0147$ & $0.0214$ &$0.0409$ & $0.0157$ & $0.0252$ & $0.0359$ & $0.0211$ & $0.0288$ & $0.0409$ & $0.0146$ & $0.0155$ & $0.0167$ & $0.0211$ & $0.0197$ & $0.0187$ & $0.0206$ & $0.0155$ & $0.0146$ & $0.0170$
    \\
    CO-SLAM~\cite{coslam}& $0.0090$ & $0.0105$ & $\textbf{0.0117}$ & $\textbf{0.0107}$ & $0.0095$ & $0.0115$ & $0.0093$ & $0.0106$ & $0.0103$ & $0.0102$ & $0.0098$ & $0.0117$ & $0.0116$ & $\textbf{0.0111}$ & $0.0109$ & $0.0106$ & $0.0111$ & $0.0095$ & $0.0097$
    \\
 GO-SLAM~\cite{zhang2023goslam} & $0.0046$ & $0.0363$  & $0.2213$ & $0.0130$ & $0.0057$ & $0.0055$ & $0.0078$ & $0.0185$ & $0.0117$ & $0.0139$ & $0.0098$ & $0.1685$ & $0.2213$ & $0.0637$ & $0.0166$ & $\textbf{0.0051}$ & $\textbf{0.0052}$ & $0.0092$ & $0.0049$ 
    \\ 
    SplaTAM-S~\cite{keetha2023splatam}& $\textbf{0.0045}$ & $\textbf{0.008}F$ & {$0.045$F} & $0.0191$ & $\textbf{0.0053}$  & $\textbf{0.0052}$ & $\textbf{0.0050}$ & $\textbf{0.0058}$ & $\textbf{0.0072}$ & $\textbf{0.0044}$ & $\textbf{0.0067}$ & $\textbf{0.0062}$ & $\textbf{0.0062}$ & {$0.045$F} & $\textbf{0.0041}$ & $0.0054$ & $0.0096$ & $\textbf{0.0046}$ & $\textbf{0.0045}$  
    \\     \midrule
        \multicolumn{20}{c}{\textbf{\textit{Survival Upper-bound:}} The highest expected performance (min ATE) attainable using all advanced models.}  \\ \midrule
      min ATE  & \multirow{3}{*}{$0.0045$} & \multirow{3}{*}{${0.0061}$}   & {${0.0111}$} & ${0.0107}$ & ${0.0053}$  & ${0.0052}$ & ${0.0050}$ & ${0.0058}$ & ${0.0072}$ & ${0.0044}$ & ${0.0067}$ & ${0.0062}$ & ${0.0062}$ & {${0.0111}$} & ${0.0041}$ & ${0.0051}$ & ${0.0052}$ & ${0.0046}$ & ${0.0045}$  
    \\ \cmidrule{5-8}\cmidrule{9-12}\cmidrule{13-16}\cmidrule{17-20}
     mean(min ATE)& &  & {${0.0069}$}  &  \multicolumn{4}{c|}{0.0066}&  \multicolumn{4}{c|}{0.0060}&  \multicolumn{4}{c|}{0.0069} &  \multicolumn{4}{c}{0.0049}
    \\ 
    \bottomrule  \bottomrule
     \multicolumn{20}{l}{{\textbf{1}) We highlight the best performance, \textit{i.e.}, the lowest ATE, under each perturbation type for static and dynamic perturbation mode in \textbf{bold}. }}\\
    \multicolumn{20}{l}{{\textbf{2}) Notation $\textbf{F}$ is to denote cases where no final trajectory is generated, which may occur due to tracking loss at the initial stage or insufficient GPU memory. It is important to note  }}\\
        \multicolumn{20}{l}{{that when calculating the ATE metric for such instances, we assign a value of 1.0 for further per-setting average.}}\\
        \multicolumn{20}{l}{{\textbf{3}) As neural models can estimate the entire trajectory, we calculate ATE on the complete trajectory. Notice that a high ATE (\textit{e.g.}, $\geq$ 0.2 [m])  is typically correlated to tracking loss.}}\\
        \multicolumn{20}{l}{{However, as ORBSLAM3~\cite{orbslam3} stops to predict subsequent frames when losing track, we follow previous literature~\cite{wang2020tartanair} to present ATE calculated with tracked partial trajectory.}}\\
            \multicolumn{20}{l}{{Hence, please be aware that a direct quantitative comparison between the ATE results of classical and neural SLAM models should be handled with caution.}}\\
    \end{tabular}
}
\end{table*}

